Fine-Tuning the Odds in Bayesian Networks

This paper proposes various new analysis techniques for Bayes networks in which conditional probability tables (CPTs) may contain symbolic variables. The key idea is to exploit scalable and powerful techniques for synthesis problems in parametric Markov chains. Our techniques are applicable to arbitrarily many, possibly dependent parameters that may occur in various CPTs. This lifts the severe restrictions on parameters, e.g., by restricting the number of parametrized CPTs to one or two, or by avoiding parameter dependencies between several CPTs, in existing works for parametric Bayes networks (pBNs). We describe how our techniques can be used for various pBN synthesis problems studied in the literature such as computing sensitivity functions (and values), simple and difference parameter tuning, ratio parameter tuning, and minimal change tuning. Experiments on several benchmarks show that our prototypical tool built on top of the probabilistic model checker Storm can handle several hundreds of parameters.

==> 3d.tex <==



\begin{tikzpicture}
  \begin{axis}[
    width=8.5cm, height=7cm,
    colormap={redgreen}{color=green), color=(red)},
    colormap access=direct,
    xlabel=p, ylabel=q,
    ]

    \addplot3[surf, shader=faceted interp, domain=0:1, point meta min=0, point meta max=1, point meta={z+0.6}] {(-9375 * (1676*x*y+(-419)*x+(-1388)*y+(-28)))/(525460*x*y^2+(-2182169)*x*y+512701*x+1786540*y^2+4439980*y+7137940)};
    %\addplot3 [surf,domain=0:1,opacity=0.5,color=black] {0.3};
  \end{axis}
\end{tikzpicture}



==> images/3d.tex <==



\begin{tikzpicture}
  \begin{axis}[
    width=8.5cm, height=7cm,
    colormap={redgreen}{color=(red), color=(green)},
    colormap access=direct,
    xlabel=p, ylabel=q,
    ]

    \addplot3[surf, shader=faceted interp, domain=0:1, point meta min=0, point meta max=1, point meta={z+0.6}] {(-9375 * (1676*x*y+(-419)*x+(-1388)*y+(-28)))/(525460*x*y^2+(-2182169)*x*y+512701*x+1786540*y^2+4439980*y+7137940)};
    %\addplot3 [surf,domain=0:1,opacity=0.5,color=black] {0.3};
  \end{axis}
\end{tikzpicture}



==> latexmkrc.tex <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> related-works.tex <==
\section{Related work}
\label{sec-related-work}
%% \subsection{State-of-the-art in parametric BNs}
%%Parametric Bayesian networks have been early investigated in \cite{DBLP:conf/ecsqaru/CastilloGH95}, where the numeric propagation algorithms were adapted for symbolic computations. The authors noted that the symbolic part of the computations exponentially grows with the number of parameters. This work has been followed by \cite{DBLP:conf/aaai/CastilloGH96,DBLP:journals/tsmc/CastilloGH97}, where the authors focused the computations on the query-relevant parameters and used the sensitivity functions to get the upper and lower bounds for the marginals. In \cite{DBLP:journals/aei/CastilloGHS97} these methods were extended to the Gaussian Bayesian networks. \\
%%A counterpart method for BN sensitivity analysis was proposed in  \cite{DBLP:conf/uai/KjaerulffG00} that was inherently based on the joint-tree algorithm. This work was driven in two directions: one-way analysis, addressing the effect of single parameters, and n-way analysis, addressing the joint effect of n parameters. To make the computations more tractable, they focused n-way analysis on the case where all the parameters happen in the same clique of the junction tree. \\
%Darwiche
%%In \cite{DBLP:journals/jair/ChanD02}, the authors have considered the task of one-way sensitivity analysis and parameter tuning in BNs. The technique has been extended to multiple parameters in \cite{DBLP:conf/uai/ChanD04}; the main focus of the study has been on the parameters all happening in the same CPT. This restriction is shown to make the problem computationally easier than the general n-way sensitivity analysis, keeping it as hard as one-way for their proposed method. The same authors have proposed a distance measure in \cite{DBLP:journals/ijar/ChanD05} with the aim for bounding the deviation from the original values of the parameters in the network when tuning the parameters. \\
%%%%%%%%%Linda C. van der Gaag and Silja Renooij%%%%%%%%%
%%In \cite{DBLP:journals/tsmc/Laskey95} a measurement had been introduced to quantify the effect of changing parameters on the probability of interest. The authors in \cite{DBLP:conf/uai/GaagR01} further propose another measurement to preserve the most likely outcome of the network. They indicate the effectiveness of their analysis method on a moderately sized real-life network. To reduce the computational part, the authors investigate the general form and the properties of sensitivity functions in \cite{DBLP:journals/amai/CoupeG02,van2007sensitivity}, focusing on one-way sensitivity analysis. The latter additionally provides the application insights in the context of robustness analysis and threshold decision making.

%%%%%%%%%% Cederal networks %%%%%%%%

In \cite{DBLP:conf/ecai/BoltBR16} the authors apply the BN sensitivity functions in order to improve inference on Cederal networks \cite{DBLP:journals/ai/Cozman00}. Some tool support for inference and sensitivity analysis on Cederal networks is given in \cite{DBLP:journals/aes/ToloPB18}.

%%%%%%%%% Constrained networks %%%%%%
%%In \cite{DBLP:journals/corr/BeaumontH17} constrained Bayesian networks are investigated. These networks are similarly defined to what we call parametric Bayesian networks.

% Probsolvable
%%In \cite{DBLP:conf/ictac/BartocciKS20} a natural translation from BNs into Prob-solvable loops have been proposed, which aims at four BN-related problems including sensitivity analysis. The sensitivity part is however limited to calculate the symbolic functions, not further extended to parameter tuning problems.



==> tables/pla-oneway-precision.tex <==
\begin{table}[hbt!]
    \centering
        \caption{ Applying \emph{pproximate parameter synthesis} for BN \emph{parameter tuning} - the subclass $p_1c_1d_1$}
    \begin{tabular}{@{}|c|cc|c|c|@{}}
        \toprule
        Network & Storm &  & SamIam & Bayesserver \\
        \midrule
         & coverage\% & threshold reported & threshold reported & threshold reported \\
        \midrule
        cancer & 99.9999 & >=0.436054 & >=0.436054 & >= 0.436054421768792 \\
        earthquake & 99.99999 & >= 0.268211 & >= 0.268211 & >= 0.268211006844541 \\
        asia & 99.99999 & >= 0.294952 & >= 0.294952 & >= 0.294952147495241 \\
        sachs & 99.99999 & >= 0.97554 & >= 0.97554 & >= 0.975539734597883 \\
        alarm & 99.9999 & >= 0.362012 & >= 0.362012 & >= 0.362012134508854 \\
        barley & 0.9 & - & >= 0.956102 & >= 0.95610124817875 \\
        insurance & 99.99999 & >= 0.927801 & >= 0.927801 & >= 0.927800679454384 \\
        win95pts & 99.9999999 & <= 0.274627 & <= 0.274627 & <= 0.274626591335031 \\
        hepar2 & 99.999999 & <= 0.079602 & <= 0.079602 & <= 0.0796019827080942 \\
        hepar2 & 99.9 & infeasible& infeasible & infeasible\\
        hailfinder & 99.9999 & >= 0.832838 & >= 0.832838 & >= 0.8328381741961298 \\
        hailfinder & 99.9 & infeasible & infeasible & infeasible \\
        water & 99.99999 & <= 0.1 & <= 0.1 & <= 0.09999999999999998 \\
        andes & 99.999999 & >= 0.8 & >= 0.8 & >= 0.7999999999660568 \\
        pathfinder & 0.9 & - & <= 0.07 & <= 0.06999999999999997 \\
        \bottomrule
    \end{tabular}
\end{table}


==> tables/pla-oneway-time.tex <==
\begin{table}[hbt!]
    \centering
    \begin{tabular}{|@{}c|cc|cc@{}|}
        \toprule
        Network & Storm &  & Bayesserver &  \\ 
        \midrule
         & synthesis time & total time & tuning time & total time \\
         \midrule
        cancer & 0.001s & 0.028s & 0.0030s & 2.895s \\
        earthquake & 0.001s & 0.029s & 0.0024s & 2.834s \\
        asia & 0.001s & 0.029s & 0.0030s & 2.963s \\
        sachs & 0.002s & 0.035s & 0.0028s & 2.920s \\
        alarm & 0.016s & 0.087s & 0.0024s & 2.980s \\
        barley & TO &  & 0.0033s & 5.617s \\
        insurance & 0.838s & 1.788s & 0.0033s & 3.012s \\
        win95pts & 0.002s & 0.302s & 0.0111s & 2.964s \\
        hepar2 & 0.046s & 0.647s & 0.0027s & 3.056s \\
        hailfinder & 0.020s & 0.734s & 0.0099s & 3.456s \\
        water & 0.002s & 1.296s & 0.0035s & 3.492s \\
        andes & 5.456s & 346.056s & 0.0034s & 3.176s \\
        pathfinder & MO &  & 0.0029s & 4.260s \\
        \bottomrule
    \end{tabular}
            \caption{Performance of Storm PLA algorithm for one-way parameter tuning against Bayesserver}
\end{table}
